Combining psychoanalysis and computer science: an empirical study of the relationship between emotions and the Lacanian discourses

This research explores the interdisciplinary interaction between psychoanalysis and computer science, suggesting a mutually beneficial exchange. Indeed, psychoanalytic concepts can enrich technological applications involving unconscious, elusive aspects of the human factor, such as social media and other interactive digital platforms. Conversely, computer science, especially Artificial Intelligence (AI), can contribute quantitative concepts and methods to psychoanalysis, identifying patterns and emotional cues in human expression. In particular, this research aims to apply computer science methods to establish fundamental relationships between emotions and Lacanian discourses. Such relations are discovered in our approach via empirical investigation and statistical analysis, and are eventually validated in a theoretical (psychoanalytic) way. It is worth noting that, although emotions have been sporadically studied in Lacanian theory, to the best of our knowledge a systematic, detailed investigation of their role is missing. Such fine-grained understanding of the role of emotions can also make the identification of Lacanian discourses more effective and easy in practise. In particular, our methods indicate the emotions with highest differentiation power in terms of corresponding discourses; conversely, we identify for each discourse the most characteristic emotions it admits. As a matter of fact, we develop a method which we call Lacanian Discourse Discovery (LDD), that simplifies (via systematizing) the identification of Lacanian discourses in texts. Although the main contribution of this paper is inherently theoretical (psychoanalytic), it can also facilitate major practical applications in the realm of interactive digital systems. Indeed, our approach can be automated through Artificial Intelligence methods that effectively identify emotions (and corresponding discourses) in texts.

==> content/theoretical_framework/old/lda_10_8_24.tex <==
%%%%%%%%
Lacanian Discourse Analysis is not a system or methodology developed by Lacan himself but rather a way of utilizing Lacanian concepts to analyze texts. It is considered a subsequent attempt by scholars, especially in the psychosocial domain, to create a "system" of text analysis aligned with Lacanian psychoanalytic theory, which was originally designed for therapeutic sessions. According to [2], Lacanian Discourse Analysis involves seven elements: analyzing the unconscious through gaps and absences, exploring the relationship between speaker, agent, and truth through Lacan's four discourses, reflecting the subject's speech to uncover hidden truths, approaching unspeakable elements as encounters with the Real, and disrupting and reorganizing the text to clarify its functions. However, this paper does not aim to delve deeply into LDA but rather to use some aspects of it, particularly the four Lacanian discourses, for a specific application and goal.

One main aspect of Lacan's approach to discourse analysis, akin to what an analyst would do in sessions with clients, is that the analysis must be conducted within the context and structure of language, or the Symbolic Realm, rather than in the Imaginary (where we imagine we understand and interpret the text subjectively). While this approach is valid and practical in the psychoanalytic domain, it is challenging to apply when extracting quantitative attributes from a text for certain applications. In this work, we use Lacanian Discourse Analysis methodology in the context of Natural Language Processing (NLP) tasks (footnote: this should not be confused with Neuro-Linguistic Programming Therapy). We define careful assumptions and steps that uphold the principles of the main theory without limiting its scope when it is not used in a psychoanalytic session.

The modification of utilizing Lacanian elements is common in theoretical studies of philosophy and politics [5]. For example, the author [1] employs aspects of Lacan's work to provide a comprehensive analysis of an interview from a film, using psychoanalytic theory as a lens to explore and highlight connections and meanings within the text without imposing it as the definitive interpretation.

In the same way, we attempt such an approach with less structured rich text. Structured text, like that of a movie script written by a screenwriter for production and audience entertainment, has the advantage of allowing one to map the social, cultural, and situational factors influencing the text and the relationships between the characters. By no means should this be considered a psychoanalytic analysis of sessions but rather a new, radical approach of combining Lacanian psychoanalytic concepts in the NLP domain. This approach aims to quickly identify the four (or five) Lacanian discourses when there is no information about social or cultural factors, the gender or attributes of the subjects, or when there are no clear connections or interactions between the characters. Additionally, this method is beneficial when the text is not structured to convey information, provide knowledge, or indirectly communicate with the reader.

Our approach focuses mainly on the four elements that make up the four (or five) Lacanian discourses, as described in section AAA. We believe all these elements can be identified by understanding their characteristics, which can be extracted from Lacan's theoretical work and descriptions by Bruce Fink and Lionel [3], [4]. We used the following characteristics when assigning the Lacanian discourses to the texts we analyzed:

The master signifier \( S_1 \) could be identified by the following attributes in the text:
\begin{itemize}
    \item Has identified with or against any signifier that the subject
    \item Any identity invented for himself
    \item Composes the identity of the Speaker
    \item Repetition of an idea / something of oneself
    \item Dreams: a self-image even if it is distorted
    \item Contradictions in speech
    \item Non-sensical signifier: when the speaker delivers an idea that makes no sense by itself
\end{itemize}

The element \( S_2 \), knowledge:
\begin{itemize}
    \item Factual information that can potentially be verified
    \item An idea or information that implies the speaker is an authority in its field / related to institutional affiliation
\end{itemize}

The barred subject \( \bar{S} \) can be identified by:
\begin{itemize}
    \item Excess expression of emotions
    \item Excess questioning
    \item Contradictory content
    \item Doubt
\end{itemize}

We could characterize our approach more as an NLP task: breaking down human text or speech into smaller parts that computer programs can easily understand. By doing so, we are able to achieve:
\begin{enumerate}
    \item An easy way of discovering Lacanian discourses in short, unstructured texts like everyday dialogues.
    \item A baseline for the development of further computer-based applications.
    \item The combination of Lacanian discourse concepts with Natural Language Processing (NLP) tasks in the field of computer science.
\end{enumerate}

Based on Chapter 2 of the book [2], we present how and when our approach aligns with the seven elements of Lacanian Discourse Analysis (LDA):

Element 1:: A Lacanian Discourse Analysis would not attempt any kind of reduction to the biographies of the characters, but it would be searching out the signifying elements that do not make sense and specifying the role those nonsensical elements play on organizing and disrupting the flow of text

{\it We don't reduce or remove elements from the speakers, and we used the whole text to find the emotions (as mentioned earlier, this is an NLP task, not a psychological process). Moreover, in some cases, we were able to identify the nonsensical elements in the conversations and map them to the corresponding Lacanian Discourses.}

Element 2: Text analysis aims at how the text is structured. Points of blockage in text/conversation means nonsensical signifiers are at work. A signifier takes value by its relation with the other signifiers
{\it In assigning the discourses and emotions, we considered the context of each speaker's conversation and their nonsensical elements.}

Element 3: The unconscious is constituted at the moment the subject starts to speak and figures as "the discourse of the Other" Analysis of what is unconscious to the subject in a piece of text is an analysis of the "gaps" and "holes" where what is said at any moment presupposes that something else cannot or will not be said. The unconscious in LDA is what functions as absence in the text. The object petit a is a device to explore the orientation of the speaker around which they move in a manner that does not reduce their orientation as only being another empirically present speaker 
{\it Like Element 2 our goal was not to find unconscious elements, nor were we trying to fill any gaps or holes; we work only with the structure of then that is in front of us}

Element 4: The 4 discourses consist of a relationship between the speaker and "agent" and the kind of the "other" that is addressed by them. The agent is underpinned by a form of "truth", and each discourse there is kind of "product" of the relationship between the speaker and agent 
{\it In our approach of assigning the Discourses we tried to discover the "product" of the discourses in the dialogues and not with the "truth" as its would require lots of fantasy and assumptions}

Element 5:
In psychoanalysis we don't fill the gaps by information we believe about the analysand. The activity of speaking divides the subject between the various things they say about themselves as they address an other and the activity of speaking as such, an activity which opens up a realm of truth (Lacan 1964/1973: 139) . The analyst's task is to take the message the subjects send, and send it back in its true signification, in an inverted form; revealing some truth that was concealed in the original message

{\it TEXT TO BE ADDED HERE}

Element 6: The closest we can speak outside the discourse are the points in speech that indicate something unspeakable, something unpresentable, (these can be treated as points encounter with the Real)

{\it TEXT TO BE ADDED HERE}

Element 7: Lacan avoids a form of interpretation that aims to reveal the signified as concepts that lie submerged under the signifiers, meaning it is not hermeneutic. The interpretation:
\begin{itemize}
    \item Would not explore the horizon of meaning.
    \item Would not delve into the internal world of speakers.
\end{itemize}
If we approach a text in a hermeneutic mode, as something we can understand within our own framework (or by recognizing it as being something opposite to what we are familiar with), for Lacanians, this would betray the stance of lying on the line of the Imaginary (imagining that we interpret from outside the text). The task of the analyst is to work on the line of the Symbolic (working within the domain of the text) and to open up the text by disrupting and disorganizing it so that its functions become clearer.

{\it We should not confuse the two tasks we did: the discourse assignment and the emotions assignment; they are completely different, and one didn't influence the other}


Summarizing, when we were assigning the Discourse, we were mentally trying to find the position of the four elements in the mathemes, not to imagine what could possibly be the Lacanian Discourse in a psychoanalytic setting. We assigned the discourses based on the characteristics of some well-defined elements like the barred subject (\( \bar{S} \)), knowledge (S2), master signifier (S1), and the object petit a (\( \alpha \)). Thus, we assigned the Lacanian Discourses while working in the Symbolic Realm and not in the Imaginary realm.

On the other hand, the emotions assignment was mainly based on keywords (essentially an NLP task) and on the imagination of the assigner regarding how the speaker felt based on the conversation. This is still in line with the application of NLP and has nothing to do with the objectives of Lacanian Discourse Analysis. This is how current transformers/LLMs (ChatGPT, BERT, etc.) discover emotions: they are trained on datasets where the annotated emotions are the possible ones expressed in the text, whether identified by keywords or by the feelings inferred by the assigners (this approach would betray the stance of working in the Imaginary Realm rather than the Symbolic).

%%%%%%%
